What Will Wi-Fi 8 Be? A Primer on IEEE 802.11bn Ultra High Reliability

What will Wi-Fi 8 be? Driven by the strict requirements of emerging applications, next-generation Wi-Fi is set to prioritize Ultra High Reliability (UHR) above all. In this paper, we explore the journey towards IEEE 802.11bn UHR, the amendment that will form the basis of Wi-Fi 8. We first present new use cases calling for further Wi-Fi evolution and associated standardization, certification, and spectrum allocation efforts. We then introduce a selection of the main disruptive features envisioned for Wi-Fi 8 and their associated research challenges, resulting from the outcome of the UHR Study Group. Among those, we focus on multi access point coordination and demonstrate that it could build upon 802.11be multi-link operation to make UHR a reality in Wi-Fi 8.

==> 02-3_Regulations.tex <==
\green{\subsection{Spectrum Allocation and Usage}} 
%\subsection{mmWave Spectrum} 
\label{sec:regulations}

\st{To maintain Wi-Fi's competitiveness and support new demanding applications, it will be crucial to secure new spectrum. 
A significant step has been taken in this regard with the decision by many countries to make the band around 6\,GHz available for secondary licensed-exempt use by Wi-Fi.
The new 6\,GHz band will offer significant advantages to Wi-Fi\,6E and Wi-Fi\,7 devices, since older generations of Wi-Fi will not be able to use it. However, these benefits will diminish as devices populate the band. 
Moreover, the 6\,GHz band can only support (in best-case scenarios) up to three 320 MHz channels, and may be unable to meet the long-term needs of Wi-Fi applications. 
In addition, the adoption of the 6\,GHz spectrum in China is still uncertain, challenging the evolution of Wi-Fi towards supporting new use cases. 
Proposals for a more efficient and integrated use of the mmWave spectrum have therefore emerged alongside initial Wi-Fi \,8 standardization discussions.} 
%\bcom{If we need to save space, I would reduce this paragraph a bit. It just lists 'intentions'.}

\blue{The \emph{IEEE 802.11 Integrated mmWave Study Group (IMMW SG)}: To ensure the long-term evolution of Wi-Fi, next-generation high-end devices could also potentially operate in all three sub-7 GHz bands as well as in the mmWave realm. Indeed, there is a growing interest in better capitalizing on the up to 14 GHz of licensed-exempt spectrum available nearly worldwide in the 60 GHz bands or 5.5 GHz in the 45 GHz band in China, respectively. 
The 60 GHz band is currently used by several incumbent technologies, such as satellite, radio astronomy, and IEEE 802.11ad/ay (WiGig). However, the market adoption of WiGig has been confined to niche applications, and regulatory bodies may consider repurposing the 60 GHz band for other bandwidth-hungry technologies such as 5G and 6G. Against this background, and after initial discussions about extending the UHR scope, it was decided to create a dedicated Integrated mmWave (IMMW) SG to consider the development of a new 802.11 amendment. This will specify carrier frequency operation between 42.5 and 71 GHz, leveraging PHY/MAC functionalities of the existing Wi-Fi 7 and future Wi-Fi 8 radio interfaces for the Sub 7 GHz bands, including channelization and multi-link framework to dynamically operate additional mmWave links.}


%OLD R1
%The \emph{IEEE 802.18 mmWave Ad Hoc Group} is exploring options in the 45\,GHz and 60\,GHz bands, which respectively offer 5.5\,GHz and 14\,GHz of spectrum. The 60\,GHz band is currently used by several incumbent technologies, such as satellite, radio astronomy, and IEEE 802.11ad/ay (WiGig). 
%However, the market adoption of WiGig has been confined to niche applications, and regulatory bodies may consider repurposing the 60\,GHz band for other bandwidth-hungry technologies such as 5G and 6G. 
%Against this background, and after initial discussions in the UHR SG, it was decided to create a dedicated \emph{Integrated mmWave (IMW) SG} to develop a new 802.11 amendment specifying carrier frequency operation between 42.5 and 71\,GHz and leveraging PHY/MAC functionalities in the existing Sub 7 GHz bands and in the future IEEE 802.11bn amendment (Wi-Fi 8).

==> 0x_SecondaryChannelAccess.tex <==
\section{\blue{Secondary Channel Access (SCA)}}

\bcom{References left as text, no added to the bib. To discuss if there is room for any.}

\textcolor{blue}{The integration of wide channels, particularly the 160 and 320 MHz variants, within Wi-Fi 8 holds substantial potential for enhancing Wi-Fi capacity. While dynamic channel access mechanisms, such as preamble puncturing, adeptly manage the available spectrum in secondary channels, when the primary channel experiences congestion, all transmission processes are unavoidably delayed, irrespective of the status of the secondary channels. In response to this challenge, Wi-Fi 8 is exploring the concept of supporting Secondary Channel Access (SCA).
%
The conceived operation of Secondary Channel Access (SCA) unfolds as follows: Initially, an Access Point (AP) and its associated stations reach a consensus to utilize an auxiliary 'primary' channel, situated within one of the 20 MHz secondary channels. This auxiliary channel serves as an alternative when the primary channel becomes occupied due to transmissions from overlapping Basic Service Sets (OBSS). In such scenarios, the AP and stations detecting OBSS activity on the primary channel seamlessly transition to monitor the auxiliary primary channel. Once it is determined to be idle, they engage in standard channel contention procedures, followed by an RTS/CTS or BSRP/BRP exchange to secure the channel for data transmission. An important constraint to adhere to is that the secondary Transmission Opportunity (TXOP) duration must conclude before the initiation of the transmission that occupies the primary channel. This allows all devices within the Basic Service Set (BSS) to return to normal operations once the primary channel becomes available again. While this approach may appear intuitive, it does challenge the conventional requirement mandating the inclusion of the primary channel in all transmissions and receptions.
%
The introduction of SCA is anticipated to yield performance gains without imposing significant complexity. The extent of these gains in terms of both throughput and latency depends on the specific scenario and OBSS configuration. Preliminary studies indicate potential gains ranging from 50\% to 250\%. Importantly, these studies also demonstrate that non-SCA BSSs do not experience any adverse performance effects. While the incorporation of SCA into Wi-Fi 8 may not represent a revolutionary leap, it does hold the promise of increasing Wi-Fi performance levels at minimal cost by creating additional channel access opportunities. Nevertheless, further research is necessary to fully understand how SCA interacts with channel allocation strategies and dynamic channel access protocols, as its presence could encourage more aggressive overlapping between OBSSs. Finally, we advise to initially limit SCA to applications involving low-latency and high-priority traffic. Such traffic typically comprises sporadic and limited data volumes, making it well-suited to harness the advantages offered by secondary channel access opportunities.}

\begin{comment}
Secondary Channel Access
============================================ 

- Non-Primary Channel Utilization Follow-up
-- "a busy 20MHz primary channel prevents a STA from accessing an idle 300 MHz of remaining bandwidth"
-- Motivation: to use the available bandwidth that otherwise is wasted always the primary channel is busy.

- Thoughts on Secondary Channel Access
-- How to leverage the use of secondary channels when the primary is busy
-- Primary channel is busy from OBSS tx.
-- Contention on secondary + TXOP shorter than the end of the NAV timer on the primary.
-- Is it equivalent to have a secondary 'primary' (this is what they propose).
-- They propose HiP EDCA

- Performance evaluation of non-primary channel access
-- The authors show some gains of NPC in different scenarios.
-- They key is: "DUT UHR AP and STA pre-negotiates an auxiliary non-primary channel to temporarily switch to when they detect medium busy on a primary channel. "

- UHR Secondary Channel Access
-- Motivation regarding the waste of spectrum when using 160 or 320 MHz channels.
-- Protocol: switch, control + TXOP < NAV

- Non-Primary Channel Access
-- Auxiliary Primary Channel
-- The same as the others


\end{comment}

==> _Unused/02_WiFi7.tex <==
\section{IEEE 802.11be: State-of-the-Art Wi-Fi\,7} \label{sec:WiFi7}

As suggested by its name (IEEE 802.11be `Extremely High Throughput' or `EHT'), Wi-Fi\,7 will augment data rates to at least 30\,Gbps per AP, about four times as fast as Wi-Fi\,6. 
In the sequel, we summarize the main features introduced in the soon-to-appear Wi-Fi\,7 commercial products \cite{garcia2021ieee,CheCheDas22}. 

\subsection{Multi-link Operation (MLO)} 

Many experts point to multi-link operation (MLO) as the main novelty Wi-Fi\,7 brings to the table, allowing Wi-Fi devices to concurrently operate on multiple channels through a single connection\cite{CarGerGal22}. MLO comes in different implementations according to the number and mode of operation of the active radios: Enhanced Multi-link Single-radio (EMLSR), Simultaneous Transmit and Receive Enhanced Multi-link Multi-radio (STR EMLMR), Non-simultaneous Transmit and Receive EMLMR (NSTR EMLMR).

Recent studies showed that in scenarios devoid of contention, STR EMLMR---the most flexible MLO implementation---supports significantly higher traffic loads (and thus throughput) than single-link for a given delay requirement. However, under high load and contention, STR EMLMR devices frequently access multiple links, often blocking contending basic service sets (BSSs) and occasionally causing even larger delays than those experienced with legacy single-link \cite{CarGerGal22}. 
Future Wi-Fi standard amendments are envisioned to prevent these worst-case events.

\subsection{320\,MHz Channels and 4K-QAM Modulation} 
These two enhancements are respectively achieved by duplicating the 160\,MHz tone plan of Wi-Fi\,6 and by adding two new modulation and coding scheme (MCS) indices. While these two upgrades jointly increase the maximum nominal rates by a factor of 2.4, wide contiguous channels of 320\,MHz are only likely to be found in the newly opened 6\,GHz band. 
Moreover, the new modulation orders require very high signal-to-noise ratios that may only be achieved in line-of-sight, close-proximity links (devoid of rich scattering and thus unsuitable for using multiple spatial streams) via beamforming, with high-quality hardware and eventually mesh-based installations.

\subsection{Multiple Resource Unit (MRU) Allocation}
To increase spectral efficiency, Wi-Fi 7 allows allocating a Multiple RU (MRU) per station (STA) consisting of a selected combination of RUs. A prime example of a scenario where such a degree of flexibility may pay off is in a BSS with a small number of users. For instance with Wi-Fi 6, an AP operating on an 80 MHz channel where the secondary 20 MHz channel is occupied was only able to assign the primary 20 MHz channel to a certain STA. Wi-Fi 7 enables the same AP to also assign the available secondary 40 MHz channel to the same STA, providing a total of 60 MHz. Such extra bandwidth can be used either to transmit faster and reduce latency, or to improve reliability by enabling more robust transmissions using lower MCSs.

\subsection{Restricted Target Wake Time (R-TWT)} 
Wi-Fi\,6 target wake time (TWT) specification \cite{nurchis2019target} aims at reducing power consumption by defining specific service periods (SP) in which a device should be awake. R-TWT builds atop this feature to define non-overlapping SPs, representing an attempt to improve support of delay-sensitive and real-time applications (RTA) through scheduled transmissions. In fact, R-TWT forces Wi-Fi\,7 STAs to end ongoing communications before the start of an advertised R-TWT SP, and it also configures a quiet interval for the entire duration of the R-TWT SP to ensure that legacy STAs remain silent.



%OLD
%As suggested by its name (IEEE 802.11be `Extremely High Throughput' or `EHT'), Wi-Fi\,7 will augment data rates to at least 30\,Gbps per AP, about four times as fast as Wi-Fi\,6. 
%%With the standardization process entering the final phase and the correspondent certification activity moving already the first steps, 
%In the sequel, we summarize the main features introduced in the soon-to-appear Wi-Fi\,7 commercial products \cite{garcia2021ieee,CheCheDas22}. 

%\bcom{We are citing 11be Draft 1.5. Is 4.0 the last one?}
% Gio: Removed \cite{80211beDraft}.fr

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%\subsection{Multi-link Operation (MLO)} 

%Many experts point to multi-link operation (MLO) as the main novelty Wi-Fi\,7 brings to the table, allowing Wi-Fi devices to concurrently operate on multiple channels through a single connection \cite{CarGerKniICC2022,CarGerGal22,lopez2022multi}. MLO comes in different implementations, with the main ones summarized as follows. 

%\subsubsection*{Enhanced Multi-link Single-radio (EMLSR)} 
%With a multi-link device (MLD) listening to two or more links simultaneously, %(e.g., by splitting its multiple radios),  performing clear channel assessment, and receiving a limited type of control frames. EMLSR supports opportunistic spectrum access at a reduced cost, as it requires a single fully functional 802.11be radio plus several other low-capability radios able only to decode 802.11 control frame preambles. Upon reception of an initial control frame on one of the links, the MLD can switch to the latter and operate using all antennas.

%\subsubsection*{Enhanced Multi-link Multi-radio (EMLMR)}
%Where all radios are 802.11be-compliant and allow operating on multiple links concurrently. EMLMR is further classified into: (i) Simultaneous Transmit and Receive (STR), where simultaneous uplink and downlink is allowed over a pair of links; (ii) Non-simultaneous Transmit and Receive (NSTR), where the above is not allowed so as to prevent self-interference.

%Lastly, non-`enhanced' versions of the above modes have also been defined, where MLSR (as opposed to EMLSR) lacks the capability of performing clear channel assessment and transmission/reception on multiple links, and MLMR (as opposed to EMLMR) lacks the capability to dynamically reconfigure spatial multiplexing over multiple links. 
%\bcom{So, what is MLSR doing different from single link? Is it that it enables faster link switching at 'management' level? How that link change is agreed between AP and STA pair?}
% Gio: In my understanding, in MLO MLSR this is handled under a single association. In SLO, this may require new association. We're using similar wording as Intel's, to be on the safe side.
%\bcom{Do we need to explain the non-enhanced ones?}
% Gio: If space allows, yes. It feels weird talking about "enhanced" without mentioning the baseline.

%Recent studies showed that in scenarios devoid of contention, STR EMLMR---the most flexible MLO implementation---supports significantly higher traffic loads (and thus throughput) than single-link for a given delay requirement. However, under high load and contention, STR EMLMR devices frequently access multiple links, often blocking contending basic service sets (BSSs) and occasionally causing even larger delays than those experienced with legacy single-link \cite{CarGerKniICC2022,CarGerGal22}. 

%\subsection{320\,MHz Channels and 4K-QAM Modulation} 
%These two enhancements are respectively achieved by duplicating the 160\,MHz tone plan of Wi-Fi\,6 and by adding two new modulation and coding scheme (MCS) indices. While these two upgrades jointly increase the maximum nominal rates by a factor of 2.4, wide contiguous channels of 320\,MHz are only likely to be found in the newly opened 6\,GHz band. Moreover, the new modulation orders require very high signal-to-noise ratios that may only be achieved in line-of-sight, close-proximity links (devoid of rich scattering and thus unsuitable for using multiple spatial streams) via beamforming, with high-quality hardware and eventually mesh-based installations.

%\subsection{Allocation of Multiple Resource Units (RU)} 
%Wi-Fi\,7 allows allocating multiple RU per station (STA) for an increased spectral efficiency. A prime example of a scenario where such degree of flexibility may pay off is with a small number of users. For instance with Wi-Fi\,6, an AP operating on an 80\,MHz channel where the secondary 20\,MHz channel is occupied was only able to assign the primary 20\,MHz channel to a certain STA. Wi-Fi\,7 enables the same AP to also assign the available secondary 40\,MHz channel, with a threefold gain in spectrum utilization. 

%\subsection{Restricted Target Wake Time (R-TWT)} 
%R-TWT comes to solve an inherent issue of the default Wi-Fi\,6 target wake time (TWT) specification \cite{nurchis2019target}: the possibility of encountering ongoing transmissions when a TWT service period (SP) starts, which adds uncertainty on when the scheduled transmission will be initiated. To avoid this situation, R-TWT forces Wi-Fi\,7 STAs to end ongoing transmissions before the start of an R-TWT SP advertised by the AP. Moreover, to ensure that non-Wi-Fi\,7 STAs also remain silent, an overlapping quiet interval is also scheduled for each R-TWT SP. R-TWT offers improved latency guarantees, representing a first attempt to support delay-sensitive applications. 


==> _Unused/04_WiFi8.tex <==
\begin{figure*}
    \centering
    \includegraphics[width=0.80\textwidth]{Figures/FeaturesWiFi8.eps}
    \caption{Illustrative examples of the key features being investigated for Wi-Fi\,8.} 
   \label{fig:WiFi8Features}
\end{figure*}

\section{IEEE 802.11bn: Key Features for Wi-Fi\,8} \label{sec:WiFi8}

Wi-Fi\,8 will be the first generation aiming to improve the protocol's reliability, with a focus on service availability and delay guarantees. Three critical aspects impacting reliability in the unlicensed spectrum are being investigated: seamless connectivity, determinism, and controlled worst-case delay.
Fig.~\ref{fig:WiFi8Features} depicts examples for each, with their chief opportunities and challenges discussed in the sequel.

\subsection{\hl{Seamless Connectivity via Distributed MLO}}

%
\footnote{\hl{Add more technical details to this subsection.}}
%
Mobility support has never been a primary focus in previous Wi-Fi standards, although devices roaming between APs is a major cause of Wi-Fi link unreliability. 
The new multi-link architecture offers a high degree of flexibility, presenting a clear split between upper (multi-link level) and lower (link level) MAC functionalities, with an MLD that can be seen as an entity that controls two or more legacy APs (or STAs) each operating on a single link. 
One way to leverage this flexibility to improve mobility support in Wi-Fi\,8 is through a new \emph{distributed} MLO framework, where APs under the control of the same MLD entity can be non-co-located rather than implemented in the same physical hardware. While this approach requires coordination and communication among the different distributed APs under the same controlling multi-link instance, it creates a distributed \emph{virtual cell} where a device's mobility is seamlessly handled by ensuring multiple links are concurrently activating from different distributed APs (Fig.~2, leftmost). This approach ensures a nomadic device is connected to at least one link, de facto embedding native roaming support into MLO and significantly improving the connection's reliability.


\subsection{\hl{Determinism via PHY and MAC Enhancements}}

%
\footnote{\hl{Add more technical details to this subsection.}}
%
Wi-Fi\,8 will consider the possibility to include PHY/MAC enhancements such as hybrid automatic repeat request (HARQ) and increasing the number of supported spatial streams from 8 to 16. The use of HARQ could allow devices to combine corrupted data units with their corresponding retransmissions to increase the probability of correct decoding, reducing latency in challenging channel conditions. 
The availability of additional spatial streams could enable more users to be served simultaneously, reducing their channel access time, and provide extra degrees of freedom to mechanisms such as coordinated beamforming (discussed later in this section). 
Additionally, other features building atop TXOP sharing functionalities will potentially allow APs to share a portion of their obtained TXOPs with associated stations for transmitting uplink frames to the AP or for direct peer-to-peer communication with another station. 
The new functionalities, combined with the aforementioned R-TWT mechanisms and TXOP sharing principles, 
already promise improvements in terms of reliability. However, further enhancements may be needed to support the arrival of unexpected or event-based time-sensitive traffic during large ongoing transmissions. An interesting proposal to address this issue is the one of frame `preemption', detailed below.

\subsubsection*{Preemption by the TXOP holder} 
To implement preemption within an ongoing PPDU transmission, a new multidimensional aggregated physical layer protocol data unit (A-PPDU) design is being studied. By aggregating multiple PPDUs in both time and frequency, the TXOP holder can replace on the fly a best-effort PPDU with a time-sensitive one, interrupting the ongoing PPDU only over the necessary resource unit. For instance (see Fig.~\ref{fig:WiFi8Features}, third example), after receiving a time-sensitive packet directed to Device\,1 (URLLC), the AP interrupts the ongoing transmission to Device 2\,of PPDU\,1 (upper 80\,MHz resource unit) to transmit the new time-sensitive frame. An interesting and positive aspect of this approach is that it does not require changing the receiver design, as interrupted frames will simply be retransmitted later.

\subsubsection*{Preemption by a non-TXOP holder} 
To implement preemption when the device transmitting a time-sensitive frame is not the TXOP holder, a more challenging situation arises. In such a case, an effective preemption mechanism should aim to capture the ongoing TXOP by exploiting the temporal inter-frame spaces between transmitted PPDUs, so that the time-sensitive frame can be squeezed in at the expense of the current data exchange. Another possibility is to allocate a short guard period at the end of all scheduled TXOPs, where only devices with time-sensitive traffic will be allowed to transmit.

\subsection{Controlled Worst-Case Delay via AP Coordination}

Random access makes it difficult to provide performance guarantees, which is why Wi-Fi\,7 introduced R-TWT to reduce contention within a BSS. However, inter-BSS interactions are still governed by contention principles, even if the APs belong to the same administrative domain, making worst-case delays unpredictable. Wi-Fi\,8 is expected to address this issue by introducing multi-AP coordination to achieve greater reliability and prevent channel access contentions, especially in dense and heavily loaded environments.

To this end, new protocols and frames will be necessary for discovering and managing multi-AP groups, sharing channel and buffer state data between APs, and triggering coordinated multi-AP transmissions to minimize inter-BSS collisions and achieve a more efficient use of the spectrum through dynamic inter-AP resource management. AP coordination schemes in Wi-Fi\,8 are envisioned to leverage both over-the-air and wired signaling. These schemes will range from basic to advanced, depending on the amount of data that must be exchanged between access points and the level of implementation complexity. While it is still to be decided what aspects of the coordination mechanism will be specified by the standard and what will be left for implementation, the main schemes are expected to include the ones described in the following.

\subsubsection*{Coordinated TDMA/OFDMA} 
Two basic approaches, respectively where a TXOP is divided in slots and sequentially allocated to different APs (TDMA) and where different portions of the band are allocated to different APs (OFDMA). 

\subsubsection*{Joint transmission} 
An advanced approach, also known as \emph{distributed MIMO}, involving non-co-located APs that jointly transmit or receive data from multiple STAs. Remarkably, this approach turns neighboring APs from potential interferers to servers. However, its implementation requires designing a new distributed CSMA/CA as well as ensuring tight synchronization in time, frequency, and phase among the transmitters. Joint data processing across multiple APs also requires an out-of-band backhaul link, whether wired or wireless.

\subsubsection*{Coordinated beamforming} 
An intermediate approach where collaborative APs suppress incoming OBSS interference in the spatial domain (see Fig.~\ref{fig:WiFi8Features}, fourth example). 
With coordinated beamforming (CBF), a next-generation multi-antenna AP can use its multiple spatial degrees of freedom to multiplex its STAs and place radiation nulls to and from neighboring non-associated STAs  \cite{GerGarLop17}. This approach makes the AP and its neighboring STAs mutually \emph{invisible}, avoiding channel access contention, allowing concurrent collision-free transmissions, and improving worst-case latency as a byproduct. 
Although the specific implementation of CBF is still under discussion, it is likely to involve the following key elements: 
\begin{itemize}
    \item A control frame exchange between two or more collaborative APs to establish and maintain a coordination set. During this exchange, APs may communicate with OBSS STAs to acquire their channel state information (CSI) and configure necessary interference suppression through nulls towards a specific channel direction or subspace.
    \item A framework for dynamic and opportunistic spatial reuse, wherein a donor AP grants a transmission opportunity to an OBSS device on which the AP places a radiation null.
    \item CSI acquisition and data transmission phases, the former being necessary to design a filter for spatial multiplexing and bidirectional interference suppression, the latter to take advantage of the new spatial reuse opportunity.
\end{itemize}

While incurring a limited implementation complexity, CBF can circumvent channel contention and deliver a substantial worst-case latency reduction, as demonstrated next.

==> _Unused/06_ComplementToWiFi8.tex <==
\section{Complementary Research Direction: Integrated mmWave Operations}

To ensure the long-term evolution of Wi-Fi, next-generation devices could be operating in all three sub-7\,GHz bands as well as in the mmWave realm. 
Indeed, there is a growing interest in capitalizing on the 5.5 and 14\,GHz of spectrum available in the 45 and 60\,GHz bands, respectively. 
While mmWave bands offer plenty of additional spectrum to offload traffic---and as a by-product reduce latency and increase reliability---they also present significant challenges. 
Rapid signal attenuation, sensitivity to blockages, %(see Fig.~\ref{fig:WiFi8Features}, second example), 
antenna beam management requirements, and high power consumption have limited the commercial adoption of products like WiGig. 
% OLD In the following, we discuss three key aspects currently debated for the 802.11bn standardization.
%Lorenzo NEW: 
In the following, we discuss three key aspects for debate in the IMW SG.

\subsubsection*{Integrated vs. independent PHY design}
%OLD: One of the main points of discussion regarding Wi-Fi\,8 is whether it will adopt a physical layer (PHY) similar to the one used in Wi-Fi\,7 for operation in mmWave bands, or leverage the one currently used in IEEE 802.11ad/ay. 
% Gio NEW. Same content but more concise to save words
One important discussion point is whether to adopt a physical layer (PHY) like Wi-Fi 7 or enhance the one in IEEE 802.11ad/ay. An integrated PHY design would eliminate the need for wide channels (2.16 GHz to 8.64 GHz) used in WiGig, reducing costs and power usage. However, this introduces challenges in handling carrier offset and phase noise at mmWave frequencies. Synchronization errors increase with carrier frequency, impairing OFDM-based systems with small subcarrier spacing. To address this, bandwidth and subcarrier spacing numerology need revisiting, with flexible subcarrier spacing scaling and appropriate FFT size adjustments to avoid processing complexity growth for wider bandwidths, similar to 5G.
%Lorenzo NEW 
%One of the main points of discussion will be whether to adopt a physical layer (PHY) similar to the one used in Wi-Fi\,7, or to enhance the one currently used in IEEE 802.11ad/ay. 
%Adopting an integrated PHY design would have a positive impact on hardware, as it would eliminate the need for the extremely wide channels (from 2.16\,GHz up to 8.64\,GHz) used by WiGig products, thus avoiding expensive and power-hungry amplifiers. However, this would also introduce new challenges. 
%When operating at mmWave frequencies, properly handling carrier frequency offset and phase noise caused by fluctuations in local oscillators becomes crucial. This is because synchronization errors increase linearly with carrier frequency, leading to significant impairments in OFDM-based systems with small subcarrier spacing. To address this issue, bandwidth and subcarrier spacing numerology need to be revisited, with the latter being flexible to upscale with channel width, similar to what is applied in 5G. Additionally, the FFT size should scale accordingly to avoid exponential increases in processing complexity for wider bandwidths.

\subsubsection*{Practical throughput gains}
% Gio revised to save words
The losses from rapid signal attenuation or blockage may offset the benefits of wider bands. Operating at mmWave can lead to a significant reduction in SINR and MCS compared to sub-7 GHz operations, resulting in a logarithmic loss in achievable rates depending on the transmitter-receiver distance. At mmWave, antenna arrays are typically used for beamforming to counteract path loss, while sub-7\,GHz bands leverage multiple antennas for parallel transmission streams, linearly increasing throughput. To determine the cost-effectiveness of mmWave operations, it is crucial to quantify realistic data rates at 60\,GHz compared to existing operations in the 6\,GHz band.
%The losses due to a more rapid signal attenuation (or worse, blockage) may offset the benefits introduced by the adoption of wider bands. Depending on the distance between transmitter and receiver, operating at mmWave may incur a drastic reduction of the SINR and of the MCS employed with respect to sub-7\,GHz operations, triggering a logarithmic loss in achievable rates. 
%Additionally at mmWave, antenna arrays must typically be used to beamform and boost signals to counteract the severe path loss, whereas in sub-7\,GHz bands multiple antennas are leveraged to generate multiple parallel transmission streams, linearly increasing the throughput. 
%To assess the cost-effectiveness of mmWave operations it is crucial to quantify realistic achievable data rates at 60\,GHz compared to existing operations in the 6\,GHz band. 

\subsubsection*{Building atop the Wi-Fi\,7 multi-link framework} 
In Section~\ref{sec:WiFi7}, we discussed MLO as the key feature of Wi-Fi\,7, enabling multiple links to operate jointly through a single association in 2.4, 5, and 6\,GHz bands. The current discussion revolves around utilizing the multi-link framework as a mechanism to integrate sub-7\,GHz and mmWave channels, offering several advantages. These include dynamically activating mmWave links when propagation conditions are favorable, and leveraging sub-7\,GHz bands to exchange control information and handle normal operations. % (see Fig. \ref{fig:WiFi8Features}, second example).


==> _Unused/XX_Figure_bubbles.tex <==
\begin{figure*}
\centering
\begin{tikzpicture}

%% The Plasma colormap: https://waldyrious.net/viridis-palette-generator/
\definecolor{viridis1}{RGB}{249, 203, 53}
%\definecolor{viridis2}{RGB}{255, 255, 53}
\definecolor{viridis3}{RGB}{173, 48, 93}
\definecolor{viridis4}{RGB}{109, 24, 110}
\definecolor{viridis5}{RGB}{68, 57, 131}

% %% The viridis colormap: https://waldyrious.net/viridis-palette-generator/
% \definecolor{viridis1}{RGB}{253,231,37}
% \definecolor{viridis2}{RGB}{94,201,98}
% \definecolor{viridis3}{RGB}{33, 145, 140}
% \definecolor{viridis4}{RGB}{59, 82, 139}
% \definecolor{viridis5}{RGB}{68, 1, 84}

%   node1/.style={shape=circle, draw=viridis2, fill=viridis2, line width=2},
%   node2/.style={shape=circle, draw=viridis3, fill=viridis3, line width=2},
%   node3/.style={shape=circle, draw=viridis4, fill=viridis4, line width=2},
%   node4/.style={shape=circle, draw=viridis5, fill=viridis5, line width=2},

  \path[small mindmap,concept,text=black,concept color=viridis1,scale=0.8]
    node[concept] {\textbf{Improving Wi-Fi performance with ML}} [clockwise from=-85]
    child[concept color=viridis1,text=black]{
      node[concept]at(-2,-2.5){Core Wi-Fi features (Section \ref{sec_core})}[clockwise from=-145]
child[concept color=viridis1,text=black,grow=-160]{
        node[concept,scale=1.1]{Channel access}[clockwise from = -145]
            child [concept color=viridis4,text=white]{node[concept, scale=0.85] {\textbf{RL/DRL}: QL, DQL, PDS, DQN, DDPG, multi-agent RL}}
            child [concept color=viridis3,text=white]{node[concept, scale=0.85] {\textbf{SL}: RF, Fixed-Share, DT}}
      }
      child[concept color=viridis1,text=black,grow=-110]{
        node[concept,scale=1.1]{Link configuration}[clockwise from =-110]
            child [concept color=viridis3,text=white]{node[concept, scale=0.85] {\textbf{SL/DSL}: ANN, RF, MLP, DNN}}
            child [concept color=viridis4,text=white]{node[concept, scale=0.85] {\textbf{RL/DRL}: SLA, QL, MAB, DQN, particle filter, SARSA}}
      }
      child[concept color=viridis1,text=black,grow=-15]{
        node[concept,scale=1.1]{Frame aggregation}[clockwise from = -15]
            %child [concept color=green,text=white]{node[concept, scale=0.85] {Online learning}}
            child [concept color=viridis3,text=white]{node[concept, scale=0.85] {\textbf{SL}: RFR, RF, M5P, SVM, ANN}}
            child [concept color=viridis4,text=white]{node[concept, scale=0.85] {\textbf{RL}: $\varepsilon$-greedy policy}}
      }
      child[concept color=viridis1,text=black,grow=-65]{
        node[concept,scale=1.1]{PHY features}[clockwise from = -65]
            child [concept color=viridis3,text=white]{node[concept, scale=0.85] {\textbf{SL/DSL}: NB, NBT, J48DT, SVM, kNN, ANN, RNN, CNN, RT, GBRT, SVR}}
            child [concept color=viridis5,text=white] {node[concept, scale=0.85] {\textbf{USL}: EMA}}
      }
    }
    child[concept color=viridis1,text=black, grow=180]{
      node[concept]at(-2.5,0){Recent Wi-Fi features (Section \ref{sec_advanced})}[clockwise from=110]
      child[concept color=viridis1,text=black]{
        node[concept,scale=1.1]{MU communication}[counterclockwise from = 110]
            child  [concept color=viridis3,text=white]{node[concept, scale=0.85] {\textbf{SL/DSL}: SVM, DNN}}
            child  [concept color=viridis4,text=white]{node[concept, scale=0.85] {\textbf{RL/DRL}: MAB, QL, DQN}}
      }
      child[concept color=viridis1,text=black,grow=155]{
        node[concept,scale=1.1]{Spatial reuse}[counterclockwise from = 150]
            child [concept color=viridis3,text=white]{node[concept, scale=0.85] {\textbf{SL}: MLP}}
            child [concept color=viridis4,text=white]{node[concept, scale=0.85] {\textbf{RL}: MAB, QL}}
      }
      child[concept color=viridis1,text=black,grow=200]{
        node[concept,scale=1.1]{Channel bonding}[counterclockwise from = 185]
            child [concept color=viridis3,text=white]{node[concept, scale=0.85] {\textbf{SL}: NN, GNN}}
            child [concept color=viridis4,text=white]{node[concept, scale=0.85] {\textbf{RL/DRL}: MAB, SARSA, DQN}}
      }
      child[concept color=viridis1,text=black,grow=250]{
        node[concept,scale=1.1]{Multi-band, network MIMO, full-duplex}[counterclockwise from =240]
            child [concept color=viridis3,text=white]{node[concept, scale=0.85] {\textbf{DSL}: DNN}}
            child [concept color=viridis4,text=white]{node[concept, scale=0.85] {\textbf{DRL}: Monte-Carlo/DDPG}}
      }
       child[concept color=viridis1,text=black,grow=300]{
        node[concept,scale=1.1]{Beamforming}[counterclockwise from =280]
            child [concept color=viridis3,text=white]{node[concept, scale=0.85] {\textbf{SL/DSL}: CNN, RF, LSTM, DNN}}
            child [concept color=viridis4,text=white]{node[concept, scale=0.85] {\textbf{RL}: QL}}
      }
}
    child[concept color=viridis1,text=black, grow = -15] {
      node[concept]at(2.5,-2.5){Connectivity management (Section \ref{sec_management})}[clockwise from=95]
        child[concept color=viridis1,text=black]{
            node[concept,scale=1.1]{Channel and band selection}[clockwise from = 95]
                child [concept color=viridis4,text=white]{node[concept, scale=0.85] {\textbf{RL/DRL}: MAB, GCN, DDQN, DQL}}
                child [concept color=viridis3,text=white]{node[concept, scale=0.85] {\textbf{SL/DSL}:  LASSO, OLS, MFNN, RF, NN, LSTM}}
        }
        child[concept color=viridis1,text=black,grow=25]{
        node[concept,scale=1.1]{Traffic prediction}[clockwise from = 45]
            child [concept color=viridis3,text=white] {node[concept, scale=0.85] {\textbf{SL/DSL}: SVM, SVR, DT, DF, DRNN}}
            child [concept color=viridis5,text=white] {node[concept, scale=0.85] {\textbf{USL}: EMA}}
      }
        child[concept color=viridis1,text=black, grow=-35]{
            node[concept,scale=1.1]{Management architectures}[clockwise from =-30]
                child [concept color=viridis4,text=white]{node[concept, scale=0.85] {\textbf{DRL}: DQL}}
                child [concept color=viridis3,text=white]{node[concept, scale=0.85] {\textbf{SL}: RF}}
        }
        child[concept color=viridis1,text=black, grow=-85]{
            node[concept,scale=1.1]{Health of Wi-Fi connections}[clockwise from =-80]
                child [concept color=viridis3,text=white]{node[concept, scale=0.85] {\textbf{SL}: RF, DT, kNN, SVM, NB, NBT, MLP, REPT, ANN}}
                child [concept color=viridis5,text=white]{node[concept, scale=0.85] {\textbf{USL}: SOHMMM}}
        }
    }
    child[concept color=viridis1,text=black, grow =85] {
      node[concept]at(-1.5,2.5){Multi-hop networks (Section \ref{sec_mhop})}[clockwise from=0]
        child[concept color=viridis1,text=black, grow =60]{
            node[concept,scale=1.1]{Ad hoc networks}[clockwise from =60]
                child [concept color=viridis4,text=white]{node[concept, scale=0.85] {\textbf{RL}: QL, RL}}
        }
        child[concept color=viridis1,text=black, grow=120]{
            node[concept,scale=1.1]{Mesh networks}[clockwise from =140]
                child [concept color=viridis3,text=white]{node[concept, scale=0.85] {\textbf{SL}: SVM, NN}}
                child [concept color=viridis4,text=white]{node[concept, scale=0.85] {\textbf{RL}: QL}}
                child [concept color=viridis5,text=white]{node[concept, scale=0.85] {\textbf{USL}: k-means clustering}}
        }
        child[concept color=viridis1,text=black, grow=170]{
            node[concept,scale=1.1]{Sensor networks}[clockwise from =170]
                child [concept color=viridis3,text=white]{node[concept, scale=0.85] {\textbf{SL/DSL}: CT, DNN, SVM}}
        }
        child[concept color=viridis1,text=black, grow=235]{
            node[concept,scale=1.1]{Vehicular networks}[clockwise from =245]
                child [concept color=viridis3,text=white]{node[concept, scale=0.85] {\textbf{SL}: SVM, RF, LR}}
                child [concept color=viridis4,text=white]{node[concept, scale=0.85] {\textbf{RL, DRL}}}
        }
    }
    child[concept color=viridis1,text=black, grow =55] {
      node[concept]at(3,1){Coexistence with other technologies (Section \ref{sec_coexistence})}[clockwise from=120]
        child[concept color=viridis1,text=black]{
            node[concept,scale=1.1]{Fair channel sharing}[counterclockwise from = 110]
                child [concept color=viridis3,text=white]{node[concept, scale=0.85] {\textbf{SL/DSL}: LR, LSTM}}
                child [concept color=viridis4,text=white]{node[concept, scale=0.85] {\textbf{RL/DRL}: QL, MAB, DQN, MDP, DQL, TRPO, DDPG}}
                %child [concept color=green!80!black!80,text=white]{node[concept, scale=0.85] {GT: Kalai-Smorodinsky bargaining}}
        }
        child[concept color=viridis1,text=black, grow = 60]{
            node[concept,scale=1.1]{Network monitoring}[clockwise from =80]
                child [concept color=viridis3,text=white]{node[concept, scale=0.85] {\textbf{SL/DSL}: RF, DNN, CNN, LSTM, NNMR}}
                child [concept color=viridis4,text=white]{node[concept, scale=0.85] {\textbf{RL}: QL, fuzzy QL, double QL}}
                child [concept color=viridis5,text=white]{node[concept, scale=0.85] {\textbf{USL/DUSL}: NN, DCC}}
        }
        child[concept color=viridis1,text=black, grow=0]{
            node[concept,scale=1.1]{Signal classification}[clockwise from = 30]
                child [concept color=viridis3,text=white]{node[concept, scale=0.85] {\textbf{SL/DSL}: NN, LR, CNN, RNN, logistic regression}}
                child [concept color=viridis5,text=white]{node[concept, scale=0.85] {\textbf{USL}: K-means clustering}}
        }
        child[concept color=viridis1,text=black, grow=180]{
            node[concept,scale=1.1]{Cooperation}[clockwise from =180]
                child [concept color=viridis4,text=white]{node[concept, scale=0.85] {\textbf{RL}: TRPO, QL}}
                child [concept color=viridis3,text=white]{node[concept, scale=0.85] {\textbf{SL}: NN}}
                %child [concept color=green!100!black!80,text=white]{node[concept, scale=0.85] {Fuzzy logic}}
        }
    }
   ;
  \matrix [below right] at (current bounding box.north west) {
  %\node [shape=circle, draw=viridis2, fill=viridis2, line width=2,label=right:Deep learning] {}; \\
  \node [shape=circle, draw=viridis3, fill=viridis3, line width=2,label=right:Supervised learning] {}; \\
  \node [shape=circle, draw=viridis4, fill=viridis4, line width=2,label=right:Reinforcement learning] {}; \\
  \node [shape=circle, draw=viridis5, fill=viridis5, line width=2,label=right:Unsupervised learning] {}; \\
};
\end{tikzpicture}
\caption{Organization of the survey and classification of research areas where Wi-Fi network performance is improved with \ac{ML} according to the literature.} %The classification of \ac{ML} methods into three categories of learning (supervised, unsupervised, reinforcement) is according to~\cite{wang2020thirty}.}
 \label{fig_MLWIFI}
\vspace{-.5em}
\end{figure*}

==> _Unused/XX_FutureWork.tex <==
\section{Research directions}

%\blue{[[Optional] \textbf{Table (Perhaps to be removed to comply with the limit. This could be discussed in each reference subsection:} Opportunities and challenges for each of the key directions]} \\

As presented in Section \ref{sec:WiFi8}, the path towards Wi-Fi 8 have already identified four distinct macro areas of work. 
%Although the standardization effort will most likely focus on defining the new required features to support them, 
In addition, we believe more fundamental research should focus on studying and understanding the benefits that forthcoming Wi-Fi upgrades may bring in terms of coexistence and performance, thinking about possible existing trade-offs and novel mechanisms to boost the required KPIs.   

Among the most interesting ones, we highlight:
\begin{itemize}
    \item \textit{Throughput vs latency trade-off}: given the well-know principle that nothing comes from nothing, theoretical works able to provide an indication of the maximum achievable throughput that can be reached when to guarantee a certain level of latency and reliability in the network are required. This will help to better design the new features, understand their applicability and benefits in the different deployment scenarios together with their impact over legacy Wi-Fi devices. 
    %
    \item \textit{Smart resource allocation mechanisms}: the degrees of freedom when deciding how to transmit data has increased significantly over the years. Flexibility in the assignment of RUs, carrier frequencies, control information, links and associated mode of operation, spatial domain radiation beams, number of nulls and its spatial directions, are demanding for the implementation of more sophisticated resource allocation strategies that take into account the dynamic needs of a variety of different applications \bb{and are able to satisfy extremely tight UHR requirements}.
    %
    \item \textit{AI/ML methods and associated architecture}: with the complexity of Wi-Fi system constantly growing, together with the need to support more stringent requirements, there is the need for a increased use of AI/ML techniques and solutions. Being currently already in use in the form of proprietary implementations, typically working among devices from the same vendor, we are heading now towards the need of a more structured and harmonized application of these techniques, the definition of a more clear architecture, with standardized interfaces, and the possibility to enable the access to a wider range of data. In this context, how AI/ML techniques will then exploit the full potential of Wi-Fi 8 is of paramount importance.  
\end{itemize}


%The use of AI/ML techniques embedded to provide better operation and improved environment understanding. AI/ML can be also used to identify traffic, acting accordingly once identified.



%    \item \textit{Capacity vs Latency trade-off}: Theoretical works able to provide determine the minimum capacity that has to be sacrified to provide latency guarantees are required to guide the design of specific mechanisms.
%    \item \textit{Practical mechanisms leveraging MLO}: to maximize spectrum access opportunities over multiple channels and bands.  




%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\begin{comment}
We conclude listing the obvious ones: performance evaluation, simulation development, tests, etc. to better understand how these features perfom both individually and in combination with others.


\bcom{[Thinking] What are the open challenges to make MAPC, mmW and reliable PHY/MAC mech? Well, more than research, is to conceive practical ways to make them work in a efficient way, and show how to get performance improvements from them. In MAPC, well, we need to reduce the amount of overheads (data exchange) to make it work. mmW? What to say since 11ad and 11ay are there given the idea is to make even simpler? All is known there, the big challenge is how to use that 'fast' link when available.... Reliable mechanism may imply the redefinition of the TXOP 'structure'. For instance, leaving 'holes' where stations/other APs can place a planned transmission (instead of not transmitting as in rTWT, start transmitting but leave room for the planned tx by 'sharing' the TXOP). In this case, agreement could be still in place, and so the goal is how to plan the 'holes'. }

\vspace*{2cm}

\noindent \bcom{Some general thoughts, not (exclusively) following the previous 3 directions (which makes sense to follow). Obvious: to go beyond what will developed in the TG}
\begin{enumerate}
    \item MAPC group schedulers (MAPC)
    %
    \item mmWave: ?
    %
    \item LL Frame insertion in on-going transmission:
    %
    \item Interplay between different features
    %
    \item Understanding the performance gains of the different features, specially in terms of latency and reliability, and their 'capacity' regions
    %
    \item \textbf{Integration of AI/ML}
    %
    \item New technologies as NOMA, in-band full-duplex, etc.
    %
    \item Development of analysis and simulation tools (NS3 is clearly not going to fill that hole).
    %
    \item Coexistence in unlicensed bands
\end{enumerate}

Due to the operation in unlicensed bands to guarantee a high level of reliability (i.e., 99.000) we need to over-provisioning resources. To do that we need a) technologies able to support over-provisioning (i.e., MLO) and b) a function that given the current situation estimates as much as accurately as possible how many resources should be allocated (i.e., number of links). With MAPC the amount of over-provisioning could be reduced, but it is still required.
\end{comment}

==> _Unused/XX_Notes.tex <==
%\section*{Notes}

%\subsection*{Boris}
%[Boris] We should check what is the Wi-Fi alliance proposing... beyond IEEE 802.11 groups. They are working on a XR profile, for instance.

%\begin{enumerate}
%    \item Multi-AP cooperation (over the air)
    %
%    \item Enhanced Multi-link Operation
    %
%    \item Profiles for XR and immersive communication, including the internet of senses.
    %
%    \item Machine Learning? Digital BSS twin?
    %
%    \item Multi-band integration (mmW)
%\end{enumerate}


%\subsection*{Lore}

%OPTION 1

%Latency performance: (i) MLO alone vs MLO + CBF. Sparse vs. dense scenario.

%Latency. Reliability. Add fast fading? [Google Stadia traffic] Multi-user MIMO?

%[1 Table with system parameters]

%[1 Figure with Latency performance]

%OPTION 2 [Lore]

%Highlight the expected shortcomings of Wi-Fi 7, in particular of MLO, with results (possible with current simulator and with reduced effort, it is just a matter of defining the most challenging scenarios for MLO). 

%Then, highlight possible strategies to overcome the expected shortcomings of Wi-Fi 7, especially focusing on latency and reliability. 



